The non-Archimedean Nirgendsnegativsemidefinitheitsstellensatz is not true

Klep and Schweighofer asked whether the Nirgendsnegativsemide-finitheitsstellensatz holds for a symmetric noncommutative polynomial whose evaluations at bounded self-adjoint operators on any nontrivial Hilbert space are not negative semidefinite. We provide an example to show the open problem has a negative answer.

==> ijmart.tex <==
%%% ====================================================================
%%%  @BibTeX-style-file{
%%%     filename        = "ijmart.bst",
%%%     copyright       = "Copyright 1995 American Mathematical Society,
%%%                        2005 The Hebrew University Magnes Press (changes)
%%%                        all rights reserved.  Copying of this file is
%%%                        authorized only if either:
%%%                        (1) you make absolutely no changes to your copy,
%%%                        including name; OR
%%%                        (2) if you do make changes, you first rename it
%%%                        to some other name.",
%%%     abstract        = "BibTeX bibliography style `ijmart' for BibTeX
%%%                        versions 0.99a or later and LaTeX version 2e.
%%%                        Produces numeric-label bibliography items in
%%%                        a form typical for the Israel journal of
%%%                        Mathematics.  The style is based on amsplain.bst
%%%
%%%  }
%%% ====================================================================

% See the file btxbst.doc for extra documentation other than
% what is included here.  And see btxhak.tex for a description
% of the BibTeX language and how to use it.

% This defines the types of fields that can occur in a database entry
% for this particular bibliography style.  Except for `language',
% this is the standard list from plain.bst.

%% Types of entries currently allowed in a BibTeX file:
%%
%% ARTICLE -- An article from a journal or magazine.
%%
%% BOOK -- A book with an explicit publisher.
%%
%% BOOKLET -- A work that is printed and bound,
%% but without a named publisher or sponsoring institution.
%%
%% CONFERENCE -- The same as INPROCEEDINGS,
%% included for Scribe compatibility.
%%
%% INBOOK -- A part of a book,
%% which may be a chapter (or section or whatever) and/or a range of pages.
%%
%% INCOLLECTION -- A part of a book having its own title.
%%
%% INPROCEEDINGS -- An article in a conference proceedings.
%%
%% MANUAL -- Technical documentation.
%%
%% MASTERSTHESIS -- A Master's thesis.
%%
%% MISC -- Use this type when nothing else fits.
%%
%% PHDTHESIS -- A PhD thesis.
%%
%% PROCEEDINGS -- The proceedings of a conference.
%%
%% TECHREPORT -- A report published by a school or other institution,
%% usually numbered within a series.
%%
%% UNPUBLISHED -- A document having an author and title, but not formally
%% published.

ENTRY
{ address
	author
	booktitle
	chapter
	edition
	editor
	howpublished
	institution
	journal
	fjournal
	key
	language
	month
	mrnumber
	note
	number
	organization
	pages
	publisher
	school
	series
	title
	type
	volume
	year
}
{}
{ label }


% Removed after.sentence, after.block---not needed.

INTEGERS { output.state before.all mid.sentence }

FUNCTION {init.state.consts}
{ #0 'before.all :=
	#1 'mid.sentence :=
}

% Scratch variables:

STRINGS { s t }

% Utility functions

FUNCTION {shows}
{ duplicate$ "::::  `" swap$ * "'" * top$
}

FUNCTION {showstack}
{"STACK====================================================================="
	top$
	stack$
	"ENDSTACK=================================================================="
	top$
}

FUNCTION {not}
{   { #0 }
	{ #1 }
	if$
}

FUNCTION {and}
{   'skip$
	{ pop$ #0 }
	if$
}

FUNCTION {or}
{   { pop$ #1 }
	'skip$
	if$
}

FUNCTION {field.or.null}
{ duplicate$ empty$
	{ pop$ "" }
	'skip$
	if$
}

FUNCTION {emphasize}
{ duplicate$ empty$
	{ pop$ "" }
	{ "\textsl{" swap$ * "}" * }
	if$
}

% n.dashify is used to make sure page ranges get the TeX code
% (two hyphens) for en-dashes.

FUNCTION {n.dashify}
{ 't :=
	""
	{ t empty$ not }
	{ t #1 #1 substring$ "-" =
		{ t #1 #2 substring$ "--" = not
			{ "--" *
				t #2 global.max$ substring$ 't :=
			}
			{   { t #1 #1 substring$ "-" = }
				{ "-" *
					t #2 global.max$ substring$ 't :=
				}
				while$
			}
			if$
		}
		{ t #1 #1 substring$ *
			t #2 global.max$ substring$ 't :=
		}
		if$
	}
	while$
}

% tie.or.space.connect connects two items with a ~ if the
% second item is less than 3 letters long, otherwise it just puts an
% ordinary space.

FUNCTION {tie.or.space.connect}
{ duplicate$ text.length$ #3 <
	{ "~" }
	{ " " }
	if$
	swap$ * *
}

FUNCTION {add.space.if.necessary}
{ duplicate$ "" =
	'skip$
	{ " " * }
	if$
}

% either.or.check gives a warning if two mutually exclusive fields
% were used in the database.

FUNCTION {either.or.check}
{ empty$
	'pop$
	{ "can't use both " swap$ * " fields in " * cite$ * warning$ }
	if$
}

% output.nonnull is called by output.

FUNCTION {output.nonnull}
% remove the top item from the stack because it's in the way.
{ 's :=
	output.state mid.sentence =
	% If we're in mid-sentence, add a comma to the new top item and write it
	{ ", " * write$ }
	% Otherwise, if we're at the beginning of a bibitem,
	{ output.state before.all =
		% just write out the top item from the stack;
		'write$
		% and the last alternative is that we're at the end of the current
		% bibitem, so we add a period to the top stack item and write it out.
		{ add.period$ " " * write$ }
		if$
		mid.sentence 'output.state :=
	}
	if$
	% Put the top item back on the stack that we removed earlier.
	s
}

% Output checks to see if the stack top is empty; if not, it
% calls output.nonnull to write it out.

FUNCTION {output}
{ duplicate$ empty$
	'pop$
	'output.nonnull
	if$
}

% Standard warning message for a missing or empty field. For the user
% we call any such field `missing' without respect to the distinction
% made by BibTeX between missing and empty.

FUNCTION {missing.warning}
{ "missing " swap$ * " in " * cite$ * warning$ }

% Output.check is like output except that it gives a warning on-screen
% if the given field in the database entry is empty.  t is the field
% name.

FUNCTION {output.check}
{ 't :=
	duplicate$ empty$
	{ pop$ t missing.warning }
	'output.nonnull
	if$
}

FUNCTION {output.bibitem}
{ newline$
	"\bibitem{" write$
		cite$ write$
		"}" write$
	newline$
	% This empty string is the first thing that will be written
	% the next time write$ is called.  Done this way because each
	% item is saved on the stack until we find out what punctuation
	% should be added after it.  Therefore we need an empty first item.
	""
	before.all 'output.state :=
}

FUNCTION {output.nonempty.mrnumber}
{ duplicate$ missing$
	{ pop$ "" }
	'skip$
	if$
	duplicate$ empty$
	'pop$
	{ " \MR{" swap$ * "}" * write$ }
	if$
}

FUNCTION {fin.entry}
{ add.period$
	write$
	mrnumber output.nonempty.mrnumber
	newline$
}

% Removed new.block, new.block.checka, new.block.checkb, new.sentence,
% new.sentence.checka, and new.sentence.checkb functions here, since they
% don't seem to be needed in the AMS style.  Also moved some real
% basic functions like `and' and 'or' earlier in the file.

INTEGERS { nameptr namesleft numnames }

% The extra section to write out a language field was added
% for AMSPLAIN.BST.  Not present in plain.bst.

FUNCTION {format.language}
{ language empty$
	{ "" }
	{ " (" language * ")" * }
	if$
}

% This version of format.names puts names in the format
%
% First von Last, Jr.
%
% (i.e., first name first, no abbreviating to initials).
% 
%  Changed by BV, 2008/01/20:  no comma before "and"


FUNCTION {format.names}
{ 's :=
	#1 'nameptr :=
	s num.names$ 'numnames :=
	numnames 'namesleft :=
	{ namesleft #0 > }
	{ s nameptr "{ff~}{vv~}{ll}{, jj}" format.name$ 't :=
		nameptr #1 >
		{ namesleft #1 >
			{ ", " * t * }
			{ numnames #3 >
				{ "," * }
				'skip$
				if$
				t "others" =
				{ " et~al." * }
				{ " and " * t * }
				if$
			}
			if$
		}
		't
		if$
		nameptr #1 + 'nameptr :=
		namesleft #1 - 'namesleft :=
	}
	while$
}

FUNCTION {format.authors}
{ author empty$
	{ "" }
	{ author format.names }
	if$
}

FUNCTION {format.editors}
{ editor empty$
	{ "" }
	{ editor format.names
		editor num.names$ #1 >
		{ " (eds.)" * }
		{ " (ed.)" * }
		if$
	}
	if$
}

FUNCTION {format.nonauthor.editors}
{ editor empty$
	{ "" }
	{ editor format.names
		editor num.names$ #1 >
		{ ", eds." * }
		{ ", ed." * }
		if$
	}
	if$
}

FUNCTION {format.title}
{ title empty$
	{ "" }
	{ title "t" change.case$ emphasize }
	if$
}

FUNCTION {format.journal.vol.year}
{ fjournal empty$
	{ journal empty$
		{ "journal name" missing.warning ""}
		{ journal }
		if$ }
	{ fjournal }
	if$
	volume empty$
	'skip$
	{ " \textbf{" * volume * "}" * }
	if$
	year empty$
	{ "year" missing.warning }
	{ " (" * year * ")" * }
	if$
}

% For formatting the issue number for a journal article.

FUNCTION {format.number}
{ number empty$
	{ "" }
	{ "no.~" number * }
	if$
}

% For formatting miscellaneous dates

FUNCTION {format.date}
{ year empty$
	{ month empty$
		{ "" }
		{ "there's a month but no year in " cite$ * warning$
			month
		}
		if$
	}
	{ month empty$
		'year
		{ month " " * year * }
		if$
	}
	if$
}

%%      The volume, series and number information is sort of tricky.
%%      This code handles it as follows:
%%      If the series is present, and the volume, but not the number,
%%        then we do "\emph{Book title}, Series Name, vol. 000"
%%      If the series is present, and the number, but not the volume,
%%        then we do "\emph{Book title}, Series Name, no. 000"
%%      If the series is present, and both number and volume,
%%        then we do "\emph{Book title}, vol. XX, Series Name, no. 000"
%%      Finally, if the series is absent,
%%        then we do "\emph{Book title}, vol. XX"
%%        or         "\emph{Book title}, no. 000"
%%        and if both volume and number are present, give a warning message.

FUNCTION {format.bookvolume.series.number}
{ volume empty$
	{ "" % Push the empty string as a placeholder in case everything else
		% is empty too.
		series empty$
		'skip$
		{ pop$ series } % if series is not empty put in stack
		if$
		number empty$
		'skip$
		{ duplicate$ empty$ % if no preceding material,
			'skip$          % do nothing, otherwise
			{ ", " * }      % add a comma and space to separate.
			if$
			"no." number tie.or.space.connect * % add the number information
		}
		if$
	}
	%% If the volume is NOT EMPTY:
	{ "vol." volume tie.or.space.connect % vol. XX
		number empty$
		{ series empty$
			'skip$
			{ series ", " * swap$ *}    % Series Name, vol. XX
			if$
		}
		{ series empty$
			{ "can't use both volume and number if series info is missing"
				warning$
				"in BibTeX entry type `" type$ * "'" * top$
			}
			{ ", " * series * ", no." * number tie.or.space.connect }
			if$
		}
		if$
	}
	if$
	
}  % end of format.bookvolume.series.number

%% format.inproc.title.where.editors is used by inproceedings entry types

%%      No case changing or emphasizing for the title.  We want initial
%%      caps, roman.
%%      We add parentheses around the address (place where conference
%%      was held).
%%      Likewise we add parentheses around the editors' names.

FUNCTION {format.inproc.title.address.editors}
{ booktitle empty$
	{ "" }
	{ booktitle
		address empty$
		'skip$
		{ add.space.if.necessary "(" * address * ")" * }
		if$
		editor empty$
		'skip$
		{ add.space.if.necessary "(" * format.nonauthor.editors * ")" * }
		if$
	}
	if$
}

%% format.incoll.title.editors is similar to format.inproc... but
%% omits the address. For collections that are not proceedings volumes.

FUNCTION {format.incoll.title.editors}
{ booktitle empty$
	{ "" }
	{ editor empty$
		{ booktitle }
		{ booktitle
			add.space.if.necessary "(" * format.nonauthor.editors * ")" *
		}
		if$
	}
	if$
}

FUNCTION {format.edition}
{ edition empty$
	{ "" }
	{ output.state mid.sentence =
		{ edition "l" change.case$ " ed." * }
		{ edition "t" change.case$ " ed." * }
		if$
	}
	if$
}

INTEGERS { multiresult }

FUNCTION {multi.page.check}
{ 't :=
	#0 'multiresult :=
	{ multiresult not
		t empty$ not
		and
	}
	{ t #1 #1 substring$
		duplicate$ "-" =
		swap$ duplicate$ "," =
		swap$ "+" =
		or or
		{ #1 'multiresult := }
		{ t #2 global.max$ substring$ 't := }
		if$
	}
	while$
	multiresult
}

FUNCTION {format.pages}
{ pages empty$
	{ "" }
	{ pages n.dashify }
	if$
}

FUNCTION {format.book.pages}
{ pages empty$
	{ "" }
	{ pages multi.page.check
		{ "pp.~" pages n.dashify * }
		{ "p.~" pages * }
		if$
	}
	if$
}

FUNCTION {format.chapter.pages}
{ chapter empty$
	'format.book.pages
	{ type empty$
		{ "ch.~" }
		{ type "l" change.case$ " " * }
		if$
		chapter *
		pages empty$
		'skip$
		{ ", " * format.book.pages * }
		if$
	}
	if$
}

FUNCTION {empty.misc.check}
{ author empty$ title empty$ howpublished empty$
	month empty$ year empty$ note empty$
	and and and and and
	key empty$ not and
	{ "all relevant fields are empty in " cite$ * warning$ }
	'skip$
	if$
}

FUNCTION {format.thesis.type}
{ type empty$
	'skip$
	{ pop$
		type "t" change.case$
	}
	if$
}

FUNCTION {format.tr.number}
{ type empty$
	{ "Tech. Report" }
	'type
	if$
	number empty$
	{ "t" change.case$ }
	{ number tie.or.space.connect }
	if$
}

% The format.crossref functions haven't been paid much attention
% at the present time (June 1990) and could probably use some
% work.  MJD

FUNCTION {format.article.crossref}
{ key empty$
	{ journal empty$
		{ "need key or journal for " cite$ * " to crossref " * crossref *
			warning$
			""
		}
		{ "in " journal * }
		if$
	}
	{ "in " key * }
	if$
	" \cite{" * crossref * "}" *
}

FUNCTION {format.crossref.editor}
{ editor #1 "{vv~}{ll}" format.name$
	editor num.names$ duplicate$
	#2 >
	{ pop$ " et~al." * }
	{ #2 <
		'skip$
		{ editor #2 "{ff }{vv }{ll}{ jj}" format.name$ "others" =
			{ " et~al." * }
			{ " and " * editor #2 "{vv~}{ll}" format.name$ * }
			if$
		}
		if$
	}
	if$
}

FUNCTION {format.book.crossref}
{ volume empty$
	{ "empty volume in " cite$ * "'s crossref of " * crossref * warning$
		"in "
	}
	{ "vol." volume tie.or.space.connect
		" of " *
	}
	if$
	editor empty$
	editor field.or.null author field.or.null =
	or
	{ key empty$
		{ series empty$
			{ "need editor, key, or series for " cite$ * " to crossref " *
				crossref * warning$
				"" *
			}
			{ series * }
			if$
		}
		{ key * }
		if$
	}
	{ format.crossref.editor * }
	if$
	" \cite{" * crossref * "}" *
}

FUNCTION {format.incoll.inproc.crossref}
{ editor empty$
	editor field.or.null author field.or.null =
	or
	{ key empty$
		{ booktitle empty$
			{ "need editor, key, or booktitle for " cite$ * " to crossref " *
				crossref * warning$
				""
			}
			{ "in \emph{" booktitle * "}" * }
			if$
		}
		{ "in " key * }
		if$
	}
	{ "in " format.crossref.editor * }
	if$
	" \cite{" * crossref * "}" *
}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% The main functions for each entry type.

% journal, vol and year are formatted together because they are
% not separated by commas.

FUNCTION {article}
{ output.bibitem
	format.authors "author" output.check
	format.title "title" output.check
	crossref missing$
	{ format.journal.vol.year output
		format.number output
		format.pages "pages" output.check
	}
	{ format.article.crossref output.nonnull
		format.pages "pages" output.check
	}
	if$
	format.language *
	note output
	fin.entry
}

FUNCTION {book}
{ output.bibitem
	author empty$
	{ format.editors "author and editor" output.check }
	{ format.authors output.nonnull
		crossref missing$
		{ "author and editor" editor either.or.check }
		'skip$
		if$
	}
	if$
	format.title "title" output.check
	format.edition output
	crossref missing$
	{ format.bookvolume.series.number output
		publisher "publisher" output.check
		address output
	}
	{ format.book.crossref output.nonnull
	}
	if$
	format.date "year" output.check
	format.language *
	note output
	fin.entry
}

FUNCTION {booklet}
{ output.bibitem
	format.authors output
	format.title "title" output.check
	howpublished output
	address output
	format.date output
	note output
	fin.entry
}

FUNCTION {inbook}
{ output.bibitem
	author empty$
	{ format.editors "author and editor" output.check }
	{ format.authors output.nonnull
		crossref missing$
		{ "author and editor" editor either.or.check }
		'skip$
		if$
	}
	if$
	format.title "title" output.check
	format.edition output
	crossref missing$
	{ format.bookvolume.series.number output
		format.chapter.pages "chapter and pages" output.check
		publisher "publisher" output.check
		address output
	}
	{ format.chapter.pages "chapter and pages" output.check
		format.book.crossref output.nonnull
	}
	if$
	format.date "year" output.check
	format.language *
	note output
	fin.entry
}

FUNCTION {incollection}
{ output.bibitem
	format.authors "author" output.check
	format.title "title" output.check
	crossref missing$
	{ format.incoll.title.editors "booktitle" output.check
		format.bookvolume.series.number output
		publisher "publisher" output.check
		address output
		format.edition output
		format.date "year" output.check
	}
	{ format.incoll.inproc.crossref output.nonnull
	}
	if$
	note output
	format.book.pages output
	format.language *
	fin.entry
}

FUNCTION {inproceedings}
{ output.bibitem
	format.authors "author" output.check
	format.title "title" output.check
	crossref missing$
	{ format.inproc.title.address.editors "booktitle" output.check
		format.bookvolume.series.number output
		organization output
		publisher output
		format.date "year" output.check
	}
	{ format.incoll.inproc.crossref output.nonnull
	}
	if$
	note output
	format.book.pages output
	format.language *
	fin.entry
}

FUNCTION {conference} { inproceedings }

FUNCTION {manual}
{ output.bibitem
	author empty$
	{ organization empty$
		'skip$
		{ organization output.nonnull
			address output
		}
		if$
	}
	{ format.authors output.nonnull }
	if$
	format.title "title" output.check
	author empty$
	{ organization empty$
		{ address output }
		'skip$
		if$
	}
	{ organization output
		address output
	}
	if$
	format.edition output
	format.date output
	note output
	fin.entry
}

FUNCTION {mastersthesis}
{ output.bibitem
	format.authors "author" output.check
	format.title "title" output.check
	"Master's thesis" format.thesis.type output.nonnull
	school "school" output.check
	address output
	format.date "year" output.check
	note output
	format.book.pages output
	fin.entry
}

FUNCTION {misc}
{ output.bibitem
	format.authors output
	format.title output
	howpublished output
	format.date output
	note output
	format.book.pages output
	fin.entry
	empty.misc.check
}

FUNCTION {phdthesis}
{ output.bibitem
	format.authors "author" output.check
	format.title "title" output.check
	"Ph.D. thesis" format.thesis.type output.nonnull
	school "school" output.check
	address output
	format.date "year" output.check
	note output
	format.book.pages output
	fin.entry
}

FUNCTION {proceedings}
{ output.bibitem
	editor empty$
	{ organization output }
	{ format.editors output.nonnull }
	if$
	format.title "title" output.check
	format.bookvolume.series.number output
	address empty$
	{ editor empty$
		'skip$
		{ organization output }
		if$
		publisher output
		format.date "year" output.check
	}
	{ address output.nonnull
		editor empty$
		'skip$
		{ organization output }
		if$
		publisher output
		format.date "year" output.check
	}
	if$
	note output
	fin.entry
}

FUNCTION {techreport}
{ output.bibitem
	format.authors "author" output.check
	format.title "title" output.check
	format.tr.number output.nonnull
	institution "institution" output.check
	address output
	format.date "year" output.check
	note output
	fin.entry
}

FUNCTION {unpublished}
{ output.bibitem
	format.authors "author" output.check
	format.title "title" output.check
	note "note" output.check
	format.date output
	fin.entry
}

FUNCTION {default.type} { misc }

MACRO {jan} {"January"}

MACRO {feb} {"February"}

MACRO {mar} {"March"}

MACRO {apr} {"April"}

MACRO {may} {"May"}

MACRO {jun} {"June"}

MACRO {jul} {"July"}

MACRO {aug} {"August"}

MACRO {sep} {"September"}

MACRO {oct} {"October"}

MACRO {nov} {"November"}

MACRO {dec} {"December"}

READ

FUNCTION {sortify}
{ purify$
	"l" change.case$
}

INTEGERS { len }

FUNCTION {chop.word}
{ 's :=
	'len :=
	s #1 len substring$ =
	{ s len #1 + global.max$ substring$ }
	's
	if$
}

FUNCTION {sort.format.names}
{ 's :=
	#1 'nameptr :=
	""
	s num.names$ 'numnames :=
	numnames 'namesleft :=
	{ namesleft #0 > }
	{ nameptr #1 >
		{ "   " * }
		'skip$
		if$
		s nameptr "{vv{ } }{ll{ }}{  ff{ }}{  jj{ }}" format.name$ 't :=
		nameptr numnames = t "others" = and
		{ "et al" * }
		{ t sortify * }
		if$
		nameptr #1 + 'nameptr :=
		namesleft #1 - 'namesleft :=
	}
	while$
}

FUNCTION {sort.format.title}
{ 't :=
	"A " #2
	"An " #3
	"The " #4 t chop.word
	chop.word
	chop.word
	sortify
	#1 global.max$ substring$
}

FUNCTION {author.sort}
{ author empty$
	{ key empty$
		{ "to sort, need author or key in " cite$ * warning$
			""
		}
		{ key sortify }
		if$
	}
	{ author sort.format.names }
	if$
}

FUNCTION {author.editor.sort}
{ author empty$
	{ editor empty$
		{ key empty$
			{ "to sort, need author, editor, or key in " cite$ * warning$
				""
			}
			{ key sortify }
			if$
		}
		{ editor sort.format.names }
		if$
	}
	{ author sort.format.names }
	if$
}

FUNCTION {author.organization.sort}
{ author empty$
	{ organization empty$
		{ key empty$
			{ "to sort, need author, organization, or key in " cite$ * warning$
				""
			}
			{ key sortify }
			if$
		}
		{ "The " #4 organization chop.word sortify }
		if$
	}
	{ author sort.format.names }
	if$
}

FUNCTION {editor.organization.sort}
{ editor empty$
	{ organization empty$
		{ key empty$
			{ "to sort, need editor, organization, or key in " cite$ * warning$
				""
			}
			{ key sortify }
			if$
		}
		{ "The " #4 organization chop.word sortify }
		if$
	}
	{ editor sort.format.names }
	if$
}

FUNCTION {presort}
{ type$ "book" =
	type$ "inbook" =
	or
	'author.editor.sort
	{ type$ "proceedings" =
		'editor.organization.sort
		{ type$ "manual" =
			'author.organization.sort
			'author.sort
			if$
		}
		if$
	}
	if$
	"    "
	*
	year field.or.null sortify
	*
	"    "
	*
	title field.or.null
	sort.format.title
	*
	#1 entry.max$ substring$
	'sort.key$ :=
}

ITERATE {presort}

SORT

STRINGS { longest.label prev.author this.author }

INTEGERS { number.label longest.label.width }

FUNCTION {initialize.longest.label}
{ "" 'longest.label :=
	#1 'number.label :=
	#0 'longest.label.width :=
	"abcxyz" 'prev.author :=
	"" 'this.author :=
}

FUNCTION {longest.label.pass}
{ number.label int.to.str$ 'label :=
	number.label #1 + 'number.label :=
	label width$ longest.label.width >
	{ label 'longest.label :=
		label width$ 'longest.label.width :=
	}
	'skip$
	if$
	author empty$
	{ editor empty$
		{ "" }
		'editor
		if$
	}
	'author
	if$
	'this.author :=
}

EXECUTE {initialize.longest.label}

ITERATE {longest.label.pass}

FUNCTION {write.lines}
{ { duplicate$ "." = NOT }
	{ write$ newline$ }
	while$
	pop$
}

FUNCTION {begin.bib}
{ preamble$ empty$
	'skip$
	{ preamble$ write$ newline$ }
	if$
	"\providecommand{\MR}{\relax\ifhmode\unskip\space\fi MR }"
	write$ newline$
	"% \MRhref is called by the amsart/book/proc definition of \MR."
	write$ newline$
	"\providecommand{\MRhref}[2]{%"
		write$ newline$
		"  \href{http://www.ams.org/mathscinet-getitem?mr=#1}{#2}"
		write$ newline$
		"}"
	write$ newline$
	"\providecommand{\href}[2]{#2}"
	write$ newline$
	"\begin{thebibliography}{"  longest.label  * "}" *
		write$ newline$
	}
	
	EXECUTE {begin.bib}
	
	EXECUTE {init.state.consts}
	
	ITERATE {call.type$}
	
	FUNCTION {end.bib}
	{ newline$
		"\end{thebibliography}" write$ newline$
}

EXECUTE {end.bib}
%% \CharacterTable
%%  {Upper-case    \A\B\C\D\E\F\G\H\I\J\K\L\M\N\O\P\Q\R\S\T\U\V\W\X\Y\Z
%%   Lower-case    \a\b\c\d\e\f\g\h\i\j\k\l\m\n\o\p\q\r\s\t\u\v\w\x\y\z
%%   Digits        \0\1\2\3\4\5\6\7\8\9
%%   Exclamation   \!     Double quote  \"     Hash (number) \#
%%   Dollar        \$     Percent       \%     Ampersand     \&
%%   Acute accent  \'     Left paren    \(     Right paren   \)
%%   Asterisk      \*     Plus          \+     Comma         \,
%%   Minus         \-     Point         \.     Solidus       \/
%%   Colon         \:     Semicolon     \;     Less than     \<
%%   Equals        \=     Greater than  \>     Question mark \?
%%   Commercial at \@     Left bracket  \[     Backslash     \\
%%   Right bracket \]     Circumflex    \^     Underscore    \_
%%   Grave accent  \`     Left brace    \{     Vertical bar  \|
%%   Right brace   \}     Tilde         \~}

